Robust Detection of Covariate-Treatment Interactions in Clinical Trials

Detection of interactions between treatment effects and patient descriptors in clinical trials is critical for optimizing the drug development process. The increasing volume of data accumulated in clinical trials provides a unique opportunity to discover new biomarkers and further the goal of personalized medicine, but it also requires innovative robust biomarker detection methods capable of detecting non-linear, and sometimes weak, signals. We propose a set of novel univariate statistical tests, based on the theory of random walks, which are able to capture non-linear and non-monotonic covariate-treatment interactions. We also propose a novel combined test, which leverages the power of all of our proposed univariate tests into a single general-case tool. We present results for both synthetic trials as well as real-world clinical trials, where we compare our method with state-of-the-art techniques and demonstrate the utility and robustness of our approach.

==> Makefile <==
FILENAME = main
PS_FILE = $(FILENAME).ps
PDF_FILE = $(FILENAME).pdf
LOG_FILE = $(FILENAME).log

PAPERSIZE = a4

LATEX_FILES = *.dvi *.log *.toc *.tof *.aux *.blg *.lof *.lot *.bbl
CLEAN_FILES = $(LATEX_FILES) *.bak core $(PS_FILE) $(PDF_FILE) *.tdo *.out *.fls *.synctex.gz *.fdb_latexmk
COMPRESS_FILES = *.tex *.bib *.sty *.eps *.ps *.fig *.m *.txt *.pgm *.bst *.cls
UNCOMPRESS_FILES = *.Z *.gz

COMPRESS_DIRS = . Tables Figures
COMPRESS = gzip -q
UNCOMPRESS = gunzip

all: main


main:
	pdflatex -jobname $(FILENAME) main
	find . -regex ".*aux" | while read auxfile; \
	do \
		if grep citation $$auxfile; then \
		echo $$auxfile >> bibbuild.log; \
		echo "------------------------" >> bibbuild.log; \
		bibtex $$auxfile >> bibbuild.log; \
		echo " " >> bibbuild.log;\
		fi; \
	done
	pdflatex -jobname $(FILENAME) main | grep Warning: > warnings.log	
	pdflatex -jobname $(FILENAME) main | grep Warning: > warnings.log

arxiv: main
	cp 
	rm *.toc
	rm *.pdf
	rm *.log
	rm *.blg
	rm *.aux


dvi2pdf:
	latex main
	@if grep "Warning: Citation" main.log; then bibtex main; \
	latex main; fi;
	@while grep Rerun main.log; do latex main; done;
	dvips -t $(PAPERSIZE) -Ppdf -j0 -G0 -o $(PS_FILE) main
	ps2pdf -sPAPERSIZE=$(PAPERSIZE) \
		-dPDFSETTINGS=/prepress \
		-dCompatibilityLevel=1.4 \
		$(PS_FILE) $(PDF_FILE)

ps: main
	dvips -t $(PAPERSIZE) -o $(PS_FILE) main

print: main
	dvips main

clean:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Cleaning $$i" ; \
	rm -f *~ ; \
	rm -f $(CLEAN_FILES) ; \
	fi) \
	done

compress: clean
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo "Compressing files in $$i" ; \
	for j in $(COMPRESS_FILES) ; \
	do \
	(if (test -f $$j) ; \
	then $(COMPRESS) $$j ; \
	fi) \
	done ; \
	fi) \
	done

uncompress:
	@for i in $(COMPRESS_DIRS) ; \
	do \
	(if (test -d $$i) ; \
	then cd $$i ; \
	echo Uncompressing files in $$i ; \
	for j in $(UNCOMPRESS_FILES) ; \
	do \
	(if (test -f $$j) ; \
	then $(UNCOMPRESS) $$j ; \
	fi) \
	done ; \
	fi) \
	done


==> tab_res_area.tex <==
{Linear}  &  \multicolumn{10}{c}{{}} \\ 
\cmidrule(lr){1-1}
{Base Coefficient} & \gudr{9.500} & \gudr{9.537} & \gudr{9.554} & \gudr{9.254} & \gudr{8.837} & \gudr{9.221} & \gudr{8.408} & \gudr{7.954} & \gudr{6.658} & \gudr{9.542}\\
{Treatment Coefficient} & 1.844 & 1.826 & 1.807 & 1.758 & 1.624 & 1.730 & 1.389 & 1.258 & 1.140 & 1.783\\
{Correlated Features} & \gudr{5.115} & \gudr{5.089} & \gudr{5.026} & 4.547 & 3.802 & 4.401 & 2.927 & 2.146 & 1.490 & 4.828\\
{Noise} & \gudr{6.276} & \gudr{6.255} & \gudr{6.302} & \gudr{6.099} & \gudr{5.432} & \gudr{5.932} & 4.813 & 3.927 & 2.917 & \gudr{6.266}\\
{Insignificant Features} & \badr{0.044} & \badr{0.044} & \badr{0.044} & \badr{0.042} & \badr{0.030} & \badr{0.038} & \badr{0.024} & \badr{0.010} & \badr{0.007} & \badr{0.041}\\
\multicolumn{11}{c}{{}}\\
{Piecewise-Smooth (3c)}  &  \multicolumn{10}{c}{{}} \\
 \cmidrule(lr){1-1}
{Noise} & 0.359 & 1.036 & 1.292 & 1.724 & 1.057 & 1.448 & 2.505 & 1.583 & 1.724 & 2.500\\
{Insignificant Features} & \badr{0.001} & \badr{0.001} & \badr{0.001} & \badr{0.003} & \badr{0.002} & \badr{0.002} & \badr{0.005} & \badr{0.003} & \badr{0.004} & \badr{0.002}\\
{Base Coefficient} & 0.104 & 0.135 & 0.172 & 0.318 & 0.276 & 0.250 & 0.583 & 0.396 & 0.370 & 0.391\\
{PC Base Coef. Positive Corr.} & 0.130 & 0.130 & 0.182 & 0.359 & 0.172 & 0.214 & 0.651 & 0.375 & 0.385 & 0.474\\
{PC Base Coef. Negative Corr.} & 0.260 & 0.302 & 0.307 & 0.474 & 0.229 & 0.422 & 0.682 & 0.333 & 0.339 & 0.344\\
\multicolumn{11}{c}{{}}\\
{Piecewise-Smooth (3r)}  &  \multicolumn{10}{c}{{}} \\
 \cmidrule(lr){1-1}
{Noise} & 2.615 & 2.698 & 2.719 & 2.750 & 4.135 & 3.510 & 2.260 & 3.469 & 2.698 & 3.651\\
{Insignificant Features} & \badr{0.005} & \badr{0.006} & \badr{0.006} & \badr{0.006} & \badr{0.016} & \badr{0.013} & \badr{0.005} & \badr{0.012} & \badr{0.007} & \badr{0.007}\\
{Base Coefficient} & 0.792 & 0.755 & 0.792 & 0.536 & 1.516 & 1.167 & 0.464 & 0.995 & 0.766 & 0.917\\
{PC Base Coef. Positive Corr.} & 0.854 & 0.891 & 0.854 & 0.875 & 1.849 & 1.474 & 0.604 & 1.219 & 0.771 & 1.036\\
{PC Base Coef. Negative Corr.} & 0.885 & 0.917 & 0.948 & 0.891 & 1.891 & 1.370 & 0.661 & 1.458 & 0.964 & 1.120\\
\multicolumn{11}{c}{{}}\\
{Piecewise-Smooth (1s)}  &  \multicolumn{10}{c}{{}} \\
 \cmidrule(lr){1-1}
{Noise} & \gudr{5.365} & \gudr{5.458} & \gudr{5.474} & \gudr{5.609} & 4.401 & \gudr{5.135} & 4.844 & 3.661 & 3.531 & \gudr{5.495}\\
{Insignificant Features} & \badr{0.032} & \badr{0.033} & \badr{0.035} & \badr{0.036} & \badr{0.019} & \badr{0.029} & \badr{0.024} & \badr{0.010} & \badr{0.010} & \badr{0.032}\\
{Base Coefficient} & 2.901 & 2.964 & 3.047 & 3.099 & 2.036 & 2.656 & 2.500 & 1.156 & 1.255 & 2.849\\
{PC Base Coef. Positive Corr.} & 2.948 & 2.974 & 3.078 & 3.141 & 1.911 & 2.719 & 2.422 & 1.099 & 1.203 & 2.750\\
{PC Base Coef. Negative Corr.} & 2.885 & 2.943 & 3.073 & 3.109 & 1.906 & 2.615 & 2.474 & 0.984 & 1.104 & 2.849\\
\multicolumn{11}{c}{{}}\\
{Piecewise-Smooth (1c)}  &  \multicolumn{10}{c}{{}} \\
 \cmidrule(lr){1-1}
{Noise} & 0.240 & 3.260 & 3.536 & 3.875 & 3.354 & 4.104 & \gudr{5.245} & 4.437 & \gudr{5.005} & \gudr{5.318}\\
{Insignificant Features} & \badr{0.001} & \badr{0.004} & \badr{0.005} & \badr{0.009} & \badr{0.008} & \badr{0.011} & \badr{0.030} & \badr{0.016} & \badr{0.024} & \badr{0.021}\\
{Base Coefficient} & 0.240 & 0.812 & 0.870 & 1.198 & 1.089 & 1.391 & 2.693 & 1.901 & 2.370 & 1.911\\
{PC Base Coef. Positive Corr.} & 0.167 & 0.693 & 0.870 & 1.260 & 0.839 & 1.307 & 2.687 & 1.786 & 2.333 & 2.042\\
{PC Base Coef. Negative Corr.} & 0.234 & 0.771 & 0.969 & 1.260 & 1.078 & 1.422 & 2.719 & 1.922 & 2.401 & 2.052\\
\multicolumn{11}{c}{{}}\\
{Piecewise-Smooth (3l)}  &  \multicolumn{10}{c}{{}} \\
 \cmidrule(lr){1-1}
{Noise} & 2.688 & 2.750 & 2.797 & 2.703 & 1.120 & 3.630 & 2.302 & 0.828 & 2.771 & 3.568\\
{Insignificant Features} & \badr{0.006} & \badr{0.006} & \badr{0.007} & \badr{0.007} & \badr{0.001} & \badr{0.011} & \badr{0.004} & \badr{0.001} & \badr{0.006} & \badr{0.009}\\
{Base Coefficient} & 0.776 & 0.740 & 0.750 & 0.724 & 0.271 & 1.250 & 0.615 & 0.349 & 0.880 & 0.807\\
{PC Base Coef. Positive Corr.} & 0.953 & 0.984 & 0.943 & 0.797 & 0.292 & 1.578 & 0.547 & 0.245 & 0.870 & 1.031\\
{PC Base Coef. Negative Corr.} & 0.885 & 0.854 & 0.875 & 0.724 & 0.281 & 1.318 & 0.568 & 0.255 & 0.948 & 1.000\\
\multicolumn{11}{c}{{}}\\
{OWL Basis}  &  \multicolumn{10}{c}{{}} \\
 \cmidrule(lr){1-1}
{noise on 78} & 0.438 & 1.349 & 1.453 & 1.555 & 1.857 & 2.333 & 3.104 & 2.583 & 3.339 & 3.003\\
{noise on 6} & 4.505 & 4.516 & 4.495 & 4.198 & 3.354 & 3.885 & 2.687 & 1.641 & 0.979 & 4.250\\
{noise on 5} & \gudr{6.984} & \gudr{6.990} & \gudr{6.990} & \gudr{6.958} & \gudr{6.911} & \gudr{6.938} & \gudr{6.391} & \gudr{6.286} & 4.813 & \gudr{6.958}\\
{noise on 3} & 0.365 & 3.396 & 3.458 & 3.385 & 4.063 & 4.583 & \gudr{5.453} & \gudr{5.198} & \gudr{5.854} & \gudr{5.370}\\
{noise on 1} & 4.484 & 4.417 & 4.349 & 3.901 & 3.682 & 4.344 & 1.375 & 1.568 & 0.474 & 4.385\\
{Insig. Features on 78} & \badr{0.001} & \badr{0.001} & \badr{0.002} & \badr{0.002} & \badr{0.005} & \badr{0.005} & \badr{0.008} & \badr{0.007} & \badr{0.010} & \badr{0.006}\\
{Insig. Features on 6} & \badr{0.018} & \badr{0.018} & \badr{0.018} & \badr{0.016} & \badr{0.009} & \badr{0.013} & \badr{0.007} & \badr{0.003} & \badr{0.003} & \badr{0.016}\\
{Insig. Features on 5} & \badr{0.049} & \badr{0.049} & \badr{0.049} & \badr{0.049} & \badr{0.049} & \badr{0.049} & \badr{0.045} & \badr{0.044} & \badr{0.020} & \badr{0.049}\\
{Insig. Features on 3} & \badr{0.001} & \badr{0.008} & \badr{0.009} & \badr{0.010} & \badr{0.016} & \badr{0.020} & \badr{0.030} & \badr{0.026} & \badr{0.035} & \badr{0.026}\\
{Insig. Features on 1} & \badr{0.018} & \badr{0.018} & \badr{0.016} & \badr{0.013} & \badr{0.012} & \badr{0.016} & \badr{0.002} & \badr{0.003} & \badr{0.001} & \badr{0.016}\\


==> tab_res_real_values_norm.tex <==
{Linear}  &  \multicolumn{10}{c}{{}} \\ 
\cmidrule(lr){1-1}
{Base Coefficient} & \gudr{0.958} & \gudr{0.979} & \gudr{0.990} & 0.896 & 0.740 & 0.896 & 0.604 & 0.542 & 0.396 & \gudr{0.990}\\
{Treatment Coefficient} & \gudr{1.000} & \gudr{0.978} & \gudr{0.957} & \gudr{0.914} & 0.774 & 0.882 & 0.527 & 0.387 & 0.258 & \gudr{0.925}\\
{Correlated Features} & \gudr{0.947} & \gudr{0.934} & 0.882 & 0.829 & 0.645 & 0.711 & 0.395 & 0.342 & 0.237 & 0.829\\
{Noise} & \gudr{0.965} & \gudr{0.965} & \gudr{0.977} & 0.884 & 0.709 & 0.860 & 0.547 & 0.337 & 0.198 & \gudr{0.930}\\
{Insignificant Features} & 0.800 & 0.863 & 0.812 & 0.637 & 0.275 & 0.562 & 0.113 & \badr{0.050} & \badr{0.037} & 0.675\\
\multicolumn{11}{c}{{}}\\
{Piecewise-Smooth (3c)}  &  \multicolumn{10}{c}{{}} \\
 \cmidrule(lr){1-1}
{Noise} & \badr{0.093} & \badr{0.093} & 0.116 & 0.419 & 0.140 & 0.233 & \gudr{0.953} & 0.419 & 0.488 & 0.837\\
{Insignificant Features} & \badr{0.000} & \badr{0.000} & \badr{0.000} & \badr{0.022} & \badr{0.000} & \badr{0.000} & \badr{0.022} & \badr{0.000} & \badr{0.000} & \badr{0.000}\\
{Base Coefficient} & \badr{0.048} & \badr{0.024} & \badr{0.071} & 0.190 & \badr{0.071} & \badr{0.095} & 0.405 & 0.167 & 0.190 & 0.286\\
{PC Base Coef. Positive Corr.} & 0.182 & 0.182 & 0.212 & 0.212 & \badr{0.091} & 0.121 & 0.455 & 0.182 & 0.152 & 0.333\\
{PC Base Coef. Negative Corr.} & 0.171 & 0.200 & 0.171 & 0.229 & 0.114 & 0.229 & 0.314 & 0.114 & \badr{0.086} & 0.229\\
\multicolumn{11}{c}{{}}\\
{Piecewise-Smooth (3r)}  &  \multicolumn{10}{c}{{}} \\
 \cmidrule(lr){1-1}
{Noise} & 0.580 & 0.614 & 0.625 & 0.693 & \gudr{1.000} & \gudr{0.909} & 0.455 & 0.886 & 0.614 & 0.898\\
{Insignificant Features} & \badr{0.045} & \badr{0.045} & \badr{0.091} & \badr{0.045} & 0.227 & 0.136 & \badr{0.068} & 0.114 & \badr{0.091} & 0.114\\
{Base Coefficient} & 0.514 & 0.486 & 0.486 & 0.270 & \gudr{0.946} & 0.865 & 0.189 & 0.541 & 0.459 & 0.757\\
{PC Base Coef. Positive Corr.} & 0.578 & 0.622 & 0.578 & 0.600 & \gudr{1.000} & 0.800 & 0.333 & 0.556 & 0.400 & 0.578\\
{PC Base Coef. Negative Corr.} & 0.622 & 0.600 & 0.644 & 0.533 & \gudr{1.000} & 0.778 & 0.333 & 0.711 & 0.400 & 0.578\\
\multicolumn{11}{c}{{}}\\
{Piecewise-Smooth (1s)}  &  \multicolumn{10}{c}{{}} \\
 \cmidrule(lr){1-1}
{Noise} & 0.815 & 0.852 & 0.852 & 0.864 & 0.543 & 0.753 & 0.691 & 0.284 & 0.259 & 0.889\\
{Insignificant Features} & 0.438 & 0.438 & 0.453 & 0.531 & \badr{0.094} & 0.438 & 0.266 & \badr{0.031} & \badr{0.016} & 0.359\\
{Base Coefficient} & \gudr{0.951} & \gudr{0.951} & \gudr{0.975} & \gudr{1.000} & 0.667 & 0.802 & 0.790 & 0.346 & 0.370 & 0.827\\
{PC Base Coef. Positive Corr.} & \gudr{0.939} & \gudr{0.927} & \gudr{0.976} & \gudr{1.000} & 0.646 & 0.890 & 0.780 & 0.427 & 0.512 & 0.805\\
{PC Base Coef. Negative Corr.} & \gudr{0.910} & \gudr{0.936} & \gudr{1.000} & \gudr{0.974} & 0.615 & 0.885 & 0.821 & 0.359 & 0.359 & 0.885\\
\multicolumn{11}{c}{{}}\\
{Piecewise-Smooth (1c)}  &  \multicolumn{10}{c}{{}} \\
 \cmidrule(lr){1-1}
{Noise} & \badr{0.013} & 0.280 & 0.333 & 0.480 & 0.400 & 0.547 & \gudr{1.000} & 0.747 & 0.880 & \gudr{0.987}\\
{Insignificant Features} & \badr{0.000} & \badr{0.000} & \badr{0.000} & \badr{0.037} & \badr{0.037} & \badr{0.019} & 0.407 & 0.111 & 0.278 & 0.167\\
{Base Coefficient} & \badr{0.060} & 0.313 & 0.328 & 0.448 & 0.403 & 0.522 & \gudr{0.985} & 0.716 & \gudr{0.925} & 0.716\\
{PC Base Coef. Positive Corr.} & \badr{0.032} & 0.222 & 0.302 & 0.476 & 0.365 & 0.492 & \gudr{0.952} & 0.651 & 0.857 & 0.841\\
{PC Base Coef. Negative Corr.} & \badr{0.068} & 0.297 & 0.392 & 0.459 & 0.486 & 0.486 & \gudr{1.000} & 0.784 & 0.865 & 0.649\\
\multicolumn{11}{c}{{}}\\
{Piecewise-Smooth (3l)}  &  \multicolumn{10}{c}{{}} \\
 \cmidrule(lr){1-1}
{Noise} & 0.566 & 0.614 & 0.614 & 0.542 & \badr{0.072} & \gudr{0.928} & 0.482 & \badr{0.036} & 0.602 & \gudr{1.000}\\
{Insignificant Features} & \badr{0.021} & \badr{0.021} & \badr{0.000} & \badr{0.000} & \badr{0.000} & \badr{0.085} & \badr{0.000} & \badr{0.000} & \badr{0.000} & \badr{0.085}\\
{Base Coefficient} & 0.457 & 0.429 & 0.457 & 0.514 & \badr{0.057} & 0.743 & 0.371 & 0.143 & 0.514 & 0.486\\
{PC Base Coef. Positive Corr.} & 0.692 & 0.692 & 0.692 & 0.538 & 0.154 & 0.846 & 0.256 & 0.128 & 0.410 & 0.615\\
{PC Base Coef. Negative Corr.} & 0.390 & 0.366 & 0.341 & 0.268 & 0.195 & 0.683 & 0.415 & 0.171 & 0.683 & 0.683\\
\multicolumn{11}{c}{{}}\\
{OWL Basis}  &  \multicolumn{10}{c}{{}} \\
 \cmidrule(lr){1-1}
{noise on 78} & \badr{0.045} & \badr{0.072} & 0.117 & 0.144 & 0.171 & 0.207 & 0.351 & 0.261 & 0.351 & 0.279\\
{noise on 6} & 0.482 & 0.464 & 0.446 & 0.375 & 0.321 & 0.446 & 0.179 & 0.125 & \badr{0.089} & 0.643\\
{noise on 5} & \gudr{1.000} & \gudr{1.000} & \gudr{1.000} & \gudr{0.990} & \gudr{0.969} & \gudr{0.969} & 0.698 & 0.667 & 0.312 & \gudr{1.000}\\
{noise on 3} & 0.102 & 0.237 & 0.220 & 0.220 & 0.424 & 0.475 & \gudr{0.915} & 0.729 & \gudr{1.000} & 0.780\\
{noise on 1} & 0.544 & 0.509 & 0.509 & 0.509 & 0.404 & 0.491 & 0.193 & 0.175 & 0.140 & 0.614\\
{Insig. Features on 78} & \badr{0.000} & \badr{0.000} & \badr{0.000} & \badr{0.000} & \badr{0.021} & \badr{0.010} & \badr{0.062} & \badr{0.031} & \badr{0.083} & \badr{0.010}\\
{Insig. Features on 6} & 0.149 & 0.170 & 0.170 & \badr{0.064} & \badr{0.021} & \badr{0.021} & \badr{0.021} & \badr{0.000} & \badr{0.000} & 0.149\\
{Insig. Features on 5} & \gudr{0.989} & \gudr{0.989} & \gudr{1.000} & \gudr{0.947} & \gudr{0.905} & \gudr{0.937} & 0.695 & 0.621 & 0.168 & \gudr{0.979}\\
{Insig. Features on 3} & \badr{0.020} & \badr{0.020} & \badr{0.020} & \badr{0.061} & 0.224 & 0.245 & 0.592 & 0.388 & 0.755 & 0.449\\
{Insig. Features on 1} & 0.204 & 0.224 & 0.224 & 0.102 & \badr{0.041} & 0.102 & \badr{0.000} & \badr{0.000} & \badr{0.000} & 0.163\\

